How Developers Engineer Test Cases: An Observational Study

One of the main challenges that developers face when testing their systems lies in engineering test cases that are good enough to reveal bugs. And while our body of knowledge on software testing and automated test case generation is already quite significant, in practice, developers are still the ones responsible for engineering test cases manually. Therefore, understanding the developers' thought- and decision-making processes while engineering test cases is a fundamental step in making developers better at testing software. In this paper, we observe 13 developers thinking-aloud while testing different real-world open-source methods, and use these observations to explain how developers engineer test cases. We then challenge and augment our main findings by surveying 72 software developers on their testing practices. We discuss our results from three different angles. First, we propose a general framework that explains how developers reason about testing. Second, we propose and describe in detail the three different overarching strategies that developers apply when testing. Third, we compare and relate our observations with the existing body of knowledge and propose future studies that would advance our knowledge on the topic.

==> tab-demographics.tex <==
\begin{table}
\caption{The demographic information of the participants in the think-aloud study (N=14).}
\label{tab:demographics}
\centering
\begin{tabular}{lrrrr}
\toprule
 & \textbf{Experience as} & \textbf{Experience} & \textbf{How often} & \\
 & \textbf{developer} & \textbf{w/JUnit}  & \textbf{write tests} & \textbf{Academic} \\
\textbf{ID} & \textbf{(in years)} & \textbf{(in years)} & \textbf{(1-5)} & \textbf{formation} \\
\midrule
P1 & 9 & 7 & 5 & BSc \\
P2 & 10 & 1.5 & 2 & BSc \\
P3 & 8 & 3 & 5 & PhD \\
P4 & 14 & 10 & 4 & BSc \\
P5 & 10 & 3 & 5 & None \\
P6 & 11 & 1 & 4 & BSc \\
P7 & 15 & 4 & 2 & BSc \\
P8 & 1 & 1 & 3 & None \\
P9 & 12 & 6 & 1 & BSc \\
P10 & 15 & 1 & 5 & BSc \\
P11 & 1 & 1 & 5 & None \\
P12 & 14 & 10 & 5 & MSc \\
P13 & 9 & 4 & 4 & BSc \\
P14 & 4.5 & 2 & 2 & BSc \\
\bottomrule
\end{tabular}
\end{table}
